Terrestrial-Satellite Spectrum Sharing in the Upper Mid-Band with Interference Nulling

The growing demand for broader bandwidth in cellular networks has turned the upper mid-band (7-24 GHz) into a focal point for expansion. However, the integration of terrestrial cellular and incumbent satellite services, particularly in the 12 GHz band, poses significant interference challenges. This paper investigates the interference dynamics in terrestrial-satellite coexistence scenarios and introduces a novel beamforming approach that leverages available ephemeris data for dynamic interference mitigation. By establishing spatial radiation nulls directed towards visible satellites, our technique ensures the protection of satellite uplink communications without markedly compromising terrestrial downlink quality. Through a practical case study, we demonstrate that our approach maintains the satellite uplink signal-to-noise ratio (SNR) degradation under 0.1 dB and incurs only a negligible SNR penalty for the terrestrial downlink. Our findings offer a promising pathway for efficient spectrum sharing in the upper mid-band, fostering a concurrent enhancement in both terrestrial and satellite network capacity.

==> 0X_discussion_elevation_angles.tex <==
\section{\red{Discussion: Effect of Elevation Angle}}

Lastly, we discuss the level of satellite interference at different elevation angles, when the BSs do not cancel the interference to the victim satellites. In such a case, we assume that the BSs perform the SVD-based transmit beamforming. 
 Fig.~\ref{fig:inr_elev_cdf} shows INR CDFs for different range of elevation angles when BSs choose the transmit beamforming vectors without considering interference nulling.

\begin{figure}[!ht]
\centering

\subfloat[][INR CDF for different elevation angles without interference nulling]
{\includegraphics[width =0.95\columnwidth]{figures/inr_elev.png} \label{fig:inr_elev_cdf}}\\
\subfloat[][PDF of elevation angles]
{\includegraphics[width =0.95\columnwidth]{figures/elev_pdf.png} \label{fig:elev_pdf}}

\caption{ INR CDF with SVD for different elevation angles of satellites and PDF of elevation angles}
\label{fig:inr_pdf_nbs10}
\end{figure}

As we discussed in \ref{sec:los_itf_channel}, when the elevation angles are lower, interference increases due to the sidelobes of the BS antenna arrays. Fig.~\ref{fig:inr_pdf_nbs10} shows the INR CDF of the satellites for different elevation angles and the probability density function (PDF) of the elevation angles of the satellites. 
As shown in Fig.~\ref{fig:inr_elev_cdf}, around $20\%$ of the transmissions yield INR$>-\SI{6}{dB}$ when $45\geq\theta\geq25$ or $65\geq\theta>45$. 
On the contrary, at a higher elevation angle $\theta > 65^\circ$, we observe the INR$>-\SI{6}{dB}$ about $2\%$ of the time. 
Fig.~\ref{fig:elev_pdf} shows the PDF of the satellite elevation angles tracked from the Starlink constellation throughout the observation time, which is consistent with the analytical result of \cite{li2002analytical}. We see that the probability of observing lower elevation angles is high, and thus LOS channels at lower elevation angles become the main interference source. 
This result implies that to save computational and tracking costs, interference nulling can be \emph{selectively}  performed only for LOS channels corresponding to lower elevation angles. 

==> XX_abstract_gio_note.tex <==
\quad\quad Gio's notes below --- please edit.
\newline

--- Setup:
\begin{itemize}
    \item 15 UEs per cell on average (can be PPP). A fraction of these UEs are UAVs, the rest are GUEs.
    \item Uplink communication. Important because it is the data-hungry direction for UAVs. Downlink command and control can be provided through sub-6GHz coverage umbrella.
    \item Choose the UAV height.
\end{itemize}

--- First experiment:
\begin{itemize}
    \item Only standard BSs.
    \item Spatial multiplexing (e.g., 2 users per cell).
    \item Increase the fraction of UAVs, e.g., as follows: 0/15, 1/15, 3/15, 5/15.
    \item Show SINR/rates as a function of the fraction of UAVs in the system. For the rates, account for the total number of users per cell, which is larger than the number of multiplexed users (Sundeep's formula).
    \item Message [TBC]: GUE performance degraded by the presence of UAVs. 
    \item (Optional) Effect of multiplexing more users per cell, effect of UAV height.
\end{itemize}

--- Second experiment:
\begin{itemize}
    \item Add rooftop cells progressively, e.g., with ISDs values as per SJ's conference paper. Same frequency band as standard cells.
    \item All UAVs associate to rooftop cells (either naturally or forced). All GUEs associate to standard cells.
    \item Show SINR/rates as a function of the fraction of UAVs in the system. For the rates, account for the total number of users per cell, which now is lower than in the first experiment.
    \item Message [TBC]: Total capacity increases for both GUEs and UAVs (win-win), reusing the same spectrum. 
    \item Message [TBC]: I need more dedicated cells if I have more UAVs in the system, meaning that I can slowly start deploying those until UAVs really proliferate.
    \item Message [TBC]: The reason for the performance improvement is ... (reduced UAV transmit power, higher UAV LoS probability, capacity gain due to the fact that GUEs only share capacity with GUEs since UAVs are served by dedicated cells, etc.)
\end{itemize}

--- Third experiment:
\begin{itemize}
    \item Confirm the above explanation on why rooftop cells improve performance.
    \item E.g., show CDF of the UAV transmit power for different values of the ISD of dedicated cells. E.g., does the power decrease as I deploy more dedicated cells?
    \item Does optimal power control further improve the performance? If so, provide intuition. What information does the optimal power control algorithm need? Can it be made more practical by only using partial information?
\end{itemize}

--- (Optional) Fourth experiment:
\begin{itemize}
    \item Reverse TDD: UAVs doing uplink to dedicated BSs while GUEs are doing downlink from standard BSs. Rationale: Since there are regulations against beamforming upwards, UAVs may as well use the whole time-frequency resources for their data-hungry uplink.
    \item Message {TBC]: The interference caused at the GUEs is tolerable, thanks to directionality and to the presence of rooftop BSs.}
\end{itemize}

--- List of Figures:
\begin{itemize}
    \item Illustration of system model
    \item SINR/rates vs number of UAVs. Optionally, show different number of streams per cell. Separate UAV/GUE SINR/rates?
    \item SINR/rates vs increasing density of rooftop cells, show different fraction of UAVs.
    \item Plot explaining why dedicated cells help, e.g., CDF of transmit power? Optional: optimal power control.
    \item (Optional) SINR of GUEs/UAVs under reverse TDD.
\end{itemize}



==> codebook_design.tex <==

\section{Codebook-based interference nulling}
\label{sec:itf_cbook}
Codebook-based precoding is vastly used in $3$GPP. In fact, modern cellular standards suggest two types of predefined codebooks, namely Type I and II, for single- and multi-user MIMO \cite{3GPP38214}. BSs may choose the best codebook matrix based on the feedback reported from the UEs or the downlink channel estimation. Since there exist no codebook implementation for interference mitigation in integrated terrestrial-satellite networks, we propose a new type of codebook that is designed to null out sidelobes that propagate upwards. Since each BS has three sectors, the beam space covered by one sector is $\mathcal {\bsym{S}} = \{(\theta, \phi) | -90^\circ \leq \theta \leq 90^\circ, -60^\circ \leq \phi \leq 60^\circ \} $, where $\theta$ and $\phi$ are the elevation and azimuth angles in the global coordinate. 
 \begin{figure}[!t]
\centering
\includegraphics[width =0.75\columnwidth]{figures/up_down_region.png}
\caption{ $\mathcal{\bsym{S}}^{\rm up}$ is the null-steering region, and $\mathcal{\bsym{S}}^{\rm down}$ is the main serving region. The global and local coordinate systems are shown via $xy$- and $x'y'$-planes}
\label{fig:regions}
\end{figure}
 Considering a minimum elevation angle to observe satellites and the downtilted angle of BSs, we define two separate beam spaces in the \emph{local coordinate system} of BSs as follows:
\begin{align}
&\bsym {\mathcal{S}}^{\rm up} = \{(\theta, \phi) | \Delta \leq \theta \leq 90^\circ + \Delta, -60^\circ \leq \phi \leq 60^\circ \} \nonumber \nonumber \\
&\bsym {\mathcal{S}}^{\rm down} = \{(\theta, \phi) | -90^\circ +\Delta \leq \theta \leq  \Delta , -60^\circ \leq \phi \leq 60^\circ \} \nonumber \nonumber
\end{align}
where $\Delta$ is downtilt angle of BSs. As shown in Fig.~\ref{fig:regions},  we want to remove the sidelobes in $\mathcal{\bsym{S}}^{\rm up}$ where the main interference channels exist, preserving the beamforming gain of the service in $\mathcal{\bsym{S}}^{\rm down}$. The direction of the downtiled antennas aligns with the $x'$ axis in the local coordinate system of a BS.

We aim to design the codebook to minimize the beamforming gain in any upper direction $(\theta, \phi) \in \bsym{\mathcal{S}}^{\rm up}$. 
In other words, given the antenna response vector $\bsym{e}(\theta_i, \phi_i )$ in a direction $(\theta_i, \phi_i) \in  \bsym{\mathcal{S}}^{\rm down}$, we create an optimal codeword $w_i$ as the solution to the following problem.
\vspace{-0.05cm}
\begin{subequations}
\begin{align}
\min \quad & \sum_{(\hat{\theta}, \hat{\phi}) \in \bsym{\mathcal{S}}^{\rm up}}\big| \bsym{e}^\Herm(\hat{\theta}, \hat{\phi})\bsym{w}_i\big|^2 \\
\textrm{s. t.} \quad & |\sqrt{N_t} - \bsym{e}^\Herm(\theta_i, \phi_i)\bsym{w}_i|^2 \leq \epsilon \\
 & \lVert \bsym{w}_i \rVert^2 = 1
\label{eq:opt_target}
\end{align}
\end{subequations}
where $(\hat{\theta}, \hat{\phi})$ can be sampled from a set of rectangular grid points, and $\epsilon$ is a tolerable gain loss. Note that $\bsym{e}(\theta_i, \phi_i )$ satisfies $\lVert \bsym{e}(\theta_i, \phi_i )\rVert^2=N_t$ as a response from the antenna array. The constraint ($3$c) indicates that each weight value in $\bsym{w}_i$ should not exceed the unit magnitude.


The problem $(3)$ is convex and easily solved with the Python convex solver \cite{diamond2016cvxpy, agrawal2018rewriting}. 
To build a codebook, we first take the steering directions from uniformly spaced discrete points in azimuth from $-60^\circ$ to $60^\circ$ and in elevation from $-5^\circ$ to $-90^\circ$ with spacing $10^\circ$, respectively, in transmission coverage $\bsym {\mathcal{S}}^{\rm down}$. The null steering codebook is created by stacking the solutions ($\bsym{w}_i$) to problem $(3)$ for each steering direction.
\begin{figure}[h]
\centering
{
\includegraphics[width=0.9\columnwidth]{figures/beam_gains.png}
}
 \caption{ Beamforming gains for $8 \times 8$ URA in the entire beam space. Null-steering area is the region where the local angle $\theta\geq\Delta$} 
 \label{fig:bf_gain}
\end{figure} 
Fig.~\ref{fig:bf_gain} shows the beamforming gains in the entire beam space when the main serving beam is steered toward the direction, $\theta = -35^\circ$ and $\phi = 40^\circ$. We observe that the gains in the null-steering space are extremely low, allowing around $2.5$ dB gain loss of transmit beamformnig. 

 

==> inteferece_nulling_cbook_old.tex <==
\section{interference-nulling codebook design}
%As shown in \cite{kang2023cellular} \cite{yastrebova2020theoretical}, without careful spectrum managements the co-channel interference of LEO satellites caused by terrestrial networks can result in severe system performance degradation. 
 %It is argued that the interference probelem caused by UEs will be solved in the similar way.

Following the suggestion of the 3GPP specification \cite{3GPP38821}, we assume that every BS uses ephemeris data to track satellite locations in real time. For example, each BS can predict the number of visible satellites, elevation angles, and distances in the time or a small time window ahead. On the basis of the information from ephemeris data, BSs are aware of in which directions they should create null-steering beams, preserving the beamforming gains to UEs. Since the beams of terrestrial BSs are steered down, they do not need to form upper-direction beams which produce interference channels to satellites.Thus, a beamforming scheme or codebook that can null out sidelobes formed in upper directions is a good choice to mitigate the interference from BSs. 

The BS has $N_{\rm RF}$ chains, each of which is connected to uniform rectangular subarrays (URA), where antennas are evenly placed by half the wavelength of the carrier frequency. Since each BS has three sectors, the beam space covered by one sector is $\mathcal {\bsym{S}} = \{(\theta, \phi) | -90^\circ \leq \theta \leq 90^\circ - \Delta, -60^\circ \leq \phi \leq 60^\circ \} $, where $\theta$ and $\phi$ are the elevation and azimuth angles in the global coordinate, and $\Delta$ are the downward angles of the antenna arrays of the BS. By ignoring the downtilted angle $\Delta$ for simplicity of analysis, two separate beam spaces are defined based on the vertical beam steering directions as follows:

\begin{align}
&\bsym {\mathcal{S}}^{\rm up} = \{(\theta, \phi) | 0^\circ \leq \theta \leq 90^\circ, -60^\circ \leq \phi \leq 60^\circ \} \nonumber \nonumber \\
&\bsym {\mathcal{S}}^{\rm down} = \{(\theta, \phi) | -90^\circ \leq \theta \leq 0^\circ , -60^\circ \leq \phi \leq 60^\circ \} \nonumber \nonumber
\end{align}

We aim to design the codebook to minimize the beamforming gain in any upper direction $(\theta, \phi) \in \bsym{\mathcal{S}}^{\rm up}$. In other words, given the antenna response vector $\bsym{e}(\theta_i, \phi_i )$ in a steering direction $(\theta_i, \phi_i) \in  \bsym{\mathcal{S}}^{\rm down}$, we want to create an optimal codeword $w_i$ by solving the following problem
\vspace{-0.05cm}
\begin{subequations}
\begin{align}
\min \quad & |\bsym{e}^H(\theta, \phi)\bsym{w}_i|^2, \quad \forall (\theta, \phi) \in \bsym{\mathcal{S}}^{\rm up} \label{eq:opt_wa} \\
\textrm{s. t.} \quad & |\sqrt{N_t} - \bsym{e}^H(\theta_i, \phi_i)\bsym{w}_i|^2 \leq \epsilon\\
  & \lVert \bsym{w}_i \rVert^2 = 1
\label{eq:opt_wb}
\end{align}

\end{subequations}
where $N_t$ is total number of antenna arrays and $\epsilon$ is a tolerable loss. The constraint ($2$c) indicates each weight value in $\bsym{w}_i$ should not exceed the unit magnitude. In the sense of implementation, the phase shifters and the amplitude attenuators control the phases and amplitudes based on each element value of $\bsym{w}_i$.

However, the optimal $\bsym{w}_i$ of the problems $(2)$ for all $(\theta, \phi) \in \bsym{\mathcal{S}}^{\rm up}$ may not produce the zero response over all null steering regions due to the constraint of gain loss (\ref{eq:opt_wb}). Therefore, we propose a codebook that can completely null out beams in a \emph{target null region}, which is defined as a part vertically dividing the entire null-steering space. Specifically, when we vertically divide the null steering space $\bsym{\mathcal{S}}^{\rm up}$ into small $N$ regions, the $l$th target region is described as
\vspace{-0.05cm}
\begin{align}
\bsym{\mathcal{S}}^{\rm up}_{N, l} = \big\{(\theta, \phi) | (l-\frac{1}{2})\Bigl\lceil{\frac{90}{N}}\Bigr\rceil &\leq \theta \leq (l+\frac{1}{2})\Bigl\lceil{\frac{90}{N}}\Bigr\rceil, \nonumber \\
-60^\circ &\leq \phi \leq 60^\circ \big\} \nonumber
\end{align}
The problems $(2)$ over the $l$th target region is approximately solved in a discrete space with the sample points $(\hat{\theta}, \hat{\phi})$  as
\vspace{-0.05cm}

\begin{subequations}
\begin{align}
\min \quad & \bigg|\sum_{(\hat{\theta}, \hat{\phi}) \in \bsym{\mathcal{S}}^{\rm up}_{N, l}} \bsym{e}^H(\hat{\theta}, \hat{\phi})\bsym{w}_i\bigg|^2 \\
\textrm{s. t.} \quad & |N_t - \bsym{e}^H(\theta_i, \phi_i)\bsym{w}_i|^2 \leq \epsilon 
\label{eq:opt_target}
\end{align}
\end{subequations}
The problems $(3)$ is convex and readily solved with the python convex solver \cite{diamond2016cvxpy, agrawal2018rewriting}. 

Fig. \ref{fig:bf_gain} (a) shows the distribution of the beamforming gains for $5\times5$ URA throughout the beam space when the main direction is $\{\theta_i = -20^\circ,~\phi_i=40^\circ\}$ and the null region is $\bsym{\mathcal{S}}^{\rm up}_{9, 5}$ We observe that the beamforming vector $\bsym{w}_i$ completely cancels out all signals in the null region, preserving the substantial gain toward the serving direction, but there still exist sidelobe gains. To reduce the gains of the formed sidelobe, we modify the target null region by adding an auxiliary null region which has a smaller spacing and solve the problem~\ref{eq:opt_target} again. For each target region, a proper auxiliary region should be combined so that the beamforming gain loss in the main direction is within the tolerable range.  

\vspace{-0.12cm}
\begin{figure}[!h]
\centering
\subfloat[]{
    \includegraphics[width=0.49\columnwidth]{figures/codebook_result_1.png}
    }
%\hspace{0.1cm}
\subfloat[]{
    \includegraphics[width=0.49\columnwidth]{figures/codebook_result_2.png}      
    }
 \caption{ Beamforming gain for $5 \times 5$ URA in the entire beam space (a) without auxiliary null region (b) with auxiliary null region} 
 \label{fig:bf_gain}
\end{figure} 
\vspace{-0.1cm}

For a null $l$ target region and an auxiliary $k$ region, we find $\bsym{w}_{i, k}$ by solving the problems $(3)$ on $\bsym{\mathcal{S}}^{\rm up}_{N, l} \bigcup \bsym {\mathcal{S}}^{\rm up}_{M, k}, (M>N)$. The optimal $\bsym{w}_{i, k^*}$ should minimize the maximum value of the sidelobe gains formed in the null steering space. Accordingly, the optimal $k^*$th auxiliary set is \textit{exhaustively} searched in the following way:
\vspace{-0.02cm}
\begin{align}
k^* = \arg\min_{1 \leq k \leq M} ~\max_{(\hat{\theta},\hat{\phi})\in \bsym{\mathcal{S}}^{\rm up}}|\bsym{w}_{i,k}^H\bsym{e}(\hat{\theta}, \hat{\phi})|^2
\label{eq:opt_k}
\end{align}
The final beamforming codeword in a steering direction $(\theta_i, \phi_i)$ becomes $\bsym{w}_{i,k^*}$. As shown in Fig. \ref{fig:bf_gain} (b), combining the auxiliary region with the target null region noticeably reduces the sidelobe gains formed in the null-steering space. 


By stacking the solutions ($\bsym{w}_i$) to problem $(3)$ and $4$ for $L$ steering directions, we build the codebook matrix completely canceling out unwanted signals in the $l$th target region denoted as $\bsym{\rm W}_l \in \bsym{C}^{N_t \times  L }$.
To do this, we first take uniformly spaced discrete points in azimuth from $-60^\circ$ to $60^\circ$ and in elevation from $0^\circ$ to $-90^\circ$ with $15^\circ$ spacing, respectively, in transmission coverage $\bsym {\mathcal{S}}^{\rm down}$. As a next step, with the given discrete steering directions, the beamforming codebook $\bsym{W}_l$ creating the $l$th target-null region is made by solving problems $3$ and $4$ for each steering direction. 

\section{Dynamic Codebook Selection over time}
We define the codebok tensor $\bsym{\mathcal{W}} \in \bsym{C}^{N \times N_t \times L}$ by stacking all the codebooks $\bsym{W}_l$ as follows. 
%covering the entire null-steering space $\bsym{\mathcal{S}}^{up}$
\begin{align}
    \bsym{\mathcal{W}} = \{\bsym{W}_1~\bsym{W}_2 \ldots \bsym{W}_N \}\nonumber
\end{align}
Using the ephemeris data, every BS tracks the elevation angles,  $\bsym{\mathcal{\theta}}(t) = \{\theta_1(t), \theta_2(t), \ldots, \theta_{N_{\rm sat}(t)}(t) \}$, corresponding to the $N_{\rm sat}(t)$ observable satellites at time $t$. To minimize interference to victim satellites, BSs should be able to choose an optimal codebook at every time among the given $N$ codebooks. Thus, we propose each BS build histogram consisting of $N$ angle bins based on the statistics of elevation angles $\bsym{\mathcal{\theta}}(t)$ and choose the optimal bin $l^*(t)$ as one having the maximum frequency number. 
\begin{align}
    l^*(t) = \arg\max_{1\leq l \leq N}{\bigg|\Big\{(l-\frac{1}{2})\Bigl\lceil{\frac{90}{N}}\Bigr\rceil \leq \theta_k(t) \leq (l+\frac{1}{2})\Bigl\lceil{\frac{90}{N}}\Bigr\rceil\Big\}\bigg|}\nonumber
\end{align}
where $k$ is the index of a satellite ($1 \leq k \leq N_{sat}(t)\nonumber$).


As long as the serving UEs are fixed over time, the BSs can keep the serving beam direction, but choose a different codebook. In other words, the optimal beamforming vector toward the steering direction $i$ at time $t$ is obtained as
\begin{align}
    w_i^*(t) = \big[\bsym{\mathcal{W}} \big]_{l^*(t),:,i} \nonumber
\end{align}
Our design reduces the implementation complexity substantially because the BSs only need to choose a different codebook over time without performing the exhaustive beam search. 

==> inteference_nulling_cbook_old2.tex <==
\section{Tracking based Interference Nulling}
Following the suggestion of the 3GPP specification \cite{3GPP38821}, we assume that every BS uses \emph{ephemeris} data to track satellite locations in real time. For example, each BS can predict the number of visible satellites, the corresponding elevation angles and distances in a time or a small time window ahead. On the basis of the information from ephemeris data, BSs are aware of in which directions they should create null-steering beams, preserving the beamforming gains to UEs.

Assume that each BS estimates a terrestrial MIMO channel $\bsym{H}_{ter}$ to an UE and tracks the azimuth and elevation angles $\{(\theta_1, \phi_1), (\theta_2, \phi_2), \ldots , (\theta_{N_{\rm sat}}, \phi_{N_{\rm sat}})\}$, of multiple satellites at the time $t$. The optimal transmit and receive beamforming vectors $w_r^*$ and $w_t^*$, are merely determined by solving the following problem with the regularized cost.
\begin{equation} \label{eq:bflam}
    {\bsym{w}}_r^*, {\bsym{w}}_t^* = \arg \max_{\bsym{w}_r, \bsym{w}_t} \left[ 
        |\bsym{w}_r^\Herm\bsym{H}_{\rm ter} \bsym{w}_t|^2 - \lambda |\bsym{w}_t^\Herm\Tilde{\bsym{H}}^\Herm|^2\right]
\end{equation}
where $\lambda>0$ is a regularization parameter, and $\Tilde{\bsym{H}} \in \bsym{C}^{N_t \times N_{\rm sat}}$ is the interference channel matrix given as $\Tilde{\bsym{H}} = \{ \bsym{e}(\theta_1, \phi_1), \bsym{e}(\theta_2, \phi_2), \ldots,  \bsym{e}(\theta_{N_{\rm sat}}, \phi_N{_{\rm sat}}) \}$. The optimal solution $\bsym{w}_r^*$ is the maximum singular vector from the singular value decomposition (SVD) of $\bsym{H}_{\rm ter}$, and $\bsym{w}_t^*$ is the maximum eigenvector of $\{\bsym{H}^\Herm_{\rm ter}\bsym{w}_r\bsym{w}_r^\Herm\bsym{H}_{\rm ter} - \lambda\Tilde{\bsym{H}}\Tilde{\bsym{H}}^\Herm \}$. 

Thus, determining the transmit beamforming vector requires calculating the maximum eigenvector over time, resulting in the time complexity $O(N_t^3)$. For ideal nullification, each BS needs to know all the multipath channels to the victim satellites and solve the problem ($2$) again.

However, estimating all the multipath channels to the victim satellites is very challenging and incurs a substantial cost.
We need to reduce the cost that occurs in each BS to cancel out interference to satellites. Hence, we propose the interference nulling codebook where each codeword creates the null-steering toward victim satellites at no calculation cost and without the need of tracking of satellites in real time. 


\section{interference-nulling Codebook Design}
%As shown in \cite{kang2023cellular} \cite{yastrebova2020theoretical}, without careful spectrum managements the co-channel interference of LEO satellites caused by terrestrial networks can result in severe system performance degradation. 
 %It is argued that the interference probelem caused by UEs will be solved in the similar way.

 Since the beams of terrestrial BSs are steered down, they do not need to form upper-direction beams which produce interference channels to satellites.Thus, a beamforming scheme or codebook that can null out sidelobes formed in upper directions is a good choice to mitigate the interference from BSs. 

The BS has $N_{\rm RF}$ chains, each of which is connected to uniform rectangular subarrays (URA), where antennas are evenly placed by half the wavelength of the carrier frequency. Since each BS has three sectors, the beam space covered by one sector is $\mathcal {\bsym{S}} = \{(\theta, \phi) | -90^\circ \leq \theta \leq 90^\circ, -60^\circ \leq \phi \leq 60^\circ \} $, where $\theta$ and $\phi$ are the elevation and azimuth angles in the global coordinate. Considering a minimum elevation angle to observe satellites and the downtilted angle of BSs, we define two separate beam spaces in the \emph{local coordinate system} of BSs as follows:
\begin{align}
&\bsym {\mathcal{S}}^{\rm up} = \{(\theta, \phi) | \Delta \leq \theta \leq 90^\circ + \Delta, -60^\circ \leq \phi \leq 60^\circ \} \nonumber \nonumber \\
&\bsym {\mathcal{S}}^{\rm down} = \{(\theta, \phi) | -90^\circ +\Delta \leq \theta \leq  \Delta , -60^\circ \leq \phi \leq 60^\circ \} \nonumber \nonumber
\end{align}
where $\Delta$ is downtilt angle of BSs. 
\begin{figure}[!h]
\centering
\includegraphics[width =0.9\columnwidth]{figures/up_down_region.png}
\caption{ $\mathcal{\bsym{S}}^{\rm up}$ is the null-steering region, and $\mathcal{\bsym{S}}^{\rm down}$ is the main serving region. The global and local coordinate systems are shown in $xy$- and $x'y'$-planes}
\label{fig:regions}
\end{figure}


As shown in Fig.~\ref{fig:regions},  we want to remove the sidelobes in $\mathcal{\bsym{S}}^{\rm up}$ where the main interference channels exist, preserving the beamforming gain of the service in $\mathcal{\bsym{S}}^{\rm down}$. The direction of the BS downtiled antennas aligns with the $x'$ axis in the local coordinate system of a BS.

We aim to design the codebook to minimize the beamforming gain in any upper direction $(\theta, \phi) \in \bsym{\mathcal{S}}^{\rm up}$. In other words, given the antenna response vector $\bsym{e}(\theta_i, \phi_i )$ in a steering direction $(\theta_i, \phi_i) \in  \bsym{\mathcal{S}}^{\rm down}$, we create an optimal codeword $w_i$ as the solution to the following problem
\vspace{-0.05cm}
\begin{subequations}
\begin{align}
\min \quad & |\bsym{e}^\Herm(\theta, \phi)\bsym{w}_i|^2, \quad \forall (\theta, \phi) \in \bsym{\mathcal{S}}^{\rm up} \label{eq:opt_wa} \\
\textrm{s. t.} \quad & |\sqrt{N_t} - \bsym{e}^\Herm(\theta_i, \phi_i)\bsym{w}_i|^2 \leq \epsilon\\
  & \lVert \bsym{w}_i \rVert^2 = 1
\label{eq:opt_wb}
\end{align}
\end{subequations}
where $N_t$ is the total number of antenna arrays and $\epsilon$ is a tolerable gain loss. Note that $\bsym{e}(\theta_i, \phi_i )$ satisfies $\lVert \bsym{e}(\theta_i, \phi_i )\rVert^2=N_t$ as a spatial signature of the antenna arrays. The constraint ($2$c) indicates that each weight value in $\bsym{w}_i$ should not exceed the unit magnitude. In the sense of implementation, the phase shifters and the amplitude attenuators control the phases and amplitudes based on each element value of $\bsym{w}_i$. The problem $(2)$ is approximately solved in a discrete space with sample points $(\hat{\theta}, \hat{\phi})$  as
\vspace{-0.05cm}
\begin{subequations}
\begin{align}
\min \quad & \sum_{(\hat{\theta}, \hat{\phi}) \in \bsym{\mathcal{S}}^{\rm up}}\big| \bsym{e}^\Herm(\hat{\theta}, \hat{\phi})\bsym{w}_i\big|^2 \\
\textrm{s. t.} \quad & |\sqrt{N_t} - \bsym{e}^\Herm(\theta_i, \phi_i)\bsym{w}_i|^2 \leq \epsilon \\
 & \lVert \bsym{w}_i \rVert^2 = 1
\label{eq:opt_target}
\end{align}
\end{subequations}
where $(\hat{\theta}, \hat{\phi})$ can be sampled from a set of rectangular grid points. 
Problem $(3)$ is convex and easily solved with the Python convex solver \cite{diamond2016cvxpy, agrawal2018rewriting}. 

To build a codebook, we first take the steering directions from uniformly spaced discrete points in azimuth from $-60^\circ$ to $60^\circ$ and in elevation from $-5^\circ$ to $-90^\circ$ with spacing $10^\circ$, respectively, in transmission coverage $\bsym {\mathcal{S}}^{\rm down}$. The null-steering codebook is made by stacking the solutions ($\bsym{w}_i$) to the problem $(3)$ for each steering direction.

\begin{figure}[!h]
\centering
{
\includegraphics[width=0.95\columnwidth]{figures/beam_gains.png}
}
 \caption{ Beamforming gains for $8 \times 8$ URA in the entire beam space. Null-steering area is the region where the local angle $\theta\geq\Delta$} 
 \label{fig:bf_gain}
\end{figure} 
Fig.~\ref{fig:bf_gain} shows the beamforming gains in the entire beam space when the main serving beam is steered toward the direction, $\theta = -35^\circ$ and $\phi = 40^\circ$. We observe that the gains in the null-steering space are extremely low, allowing around $2.5$ dB gain loss of transmit beamformnig. 

 %The right panel of Fig.~\ref{fig:inr_snr_nbs10} shows the SNR CDFs of terrestrial UEs when applying different nulling schemes. Since we assume massive MIMO ($8\times8$ URA) with the resulting higher beamforming gain, the SNR values fall within an exceptionally high range of values. 
%We see that there is no loss of SNR for tracking-based nulling which is almost the same result as using SVD. However, there exists SNR loss of  around $3$ dB in codebook-based nulling because a tolerable gain loss is allowed when solving the problem ($3$).
%\begin{figure}[!t]
%\centering
%\includegraphics[width =0.93\columnwidth]{figures/snr_10BS.png}
%\caption{SNR CDFs of terrestrial UEs in downlink scenario}
%\label{fig:snr_nbs10}
%\end{figure}

%\subsection*{Different number of Interferers}
% We evaluate the performance of interference nulling shcemes with different numbers of concurrent transmitters to control the degree of interference. Figure 8~\ref{fig:inr_snr_nbs10} shows the INR distributions for two proposed nulling schemes when increasing the number of BS transmitting simultaneously. As shown in the right panel, tracking-based nulling eliminates interference to satellites despite the high number of parallel transmissions of BSs. 

%\begin{figure}[!h]
%\centering
%\includegraphics[width =0.99\columnwidth]{figures/inr_with_diff_nBS.png}
%\caption{ distributions of INRs for two proposed beamforming schemes with the different number of concurrent transmissions}
%\label{fig:inr_snr_nbs10}
%\end{figure}


==> introduction_old.tex <==
\section{Introduction}

Traditional cellular communication networks have progressed in the last three decades from the first generation ($1$G) to the fifth generation ($5$G). However, due to economic and geographic constraints, there are still many regions, such as rural areas, where terrestrial networks may not provide good service. 
In the next cellular networks, satellite communications are expected to overcome coverage issues due to their broad coverage, speed of implementation, multicasting, and broadcast service. In particular, with multi-satellite constellations, it is possible to provide the Internet service to any location on the Earth at any time. For example, Starlink has started to provide the Internet service from more than $4600$ low Earth orbit (LEO) satellites. 

Thus, the integration of satellites and terrestrial networks has been considered a promising architecture for solving problems that terrestrial networks cannot solve \cite{kodheli2017integration,tirmizi2022hybrid,etsi2013satellite,zhu2019cooperative}. Furthermore, as increasing demand for connectivity in future cellular networks requires more spectrum usages and leads to spectrum scarcity, spectrum sharing between satellite and terrestrial networks can enhance spectrum efficiency and system capacity. Accordingly, the shared spectrum bands can be \emph{the upper mid-band} such as C-band, Ku-band, and Ka-band, which are currently assigned to satellite operators\cite{kang2023cellular}. 

However, spectrum sharing without careful network management leads to high interference to satellite service links \cite{yastrebova2020theoretical, deslandes2010analysis}. 
In particular, sidelobe transmissions due to transmit beamforming by base stations (BS) can result in the strong interference to satellite uplink since most BSs employ massive multiple antennas and transmit with relatively high power. Hence, when operating in the same frequency band, cautious transmission beamforming is indispensable to mitigate the co-channel interference.
In this work, we mainly pay attention to the transmission of BSs as the worst-case scenario.

 In prior work, there has been a limited number of endeavors to reduce sidelobe interference by BSs.
In \cite{jo2011transmit}, the transmit-nulling codebook is proposed to mitigate interference to the fixed wireless service caused by BSs that are equipped with a uniform linear array (ULA). However, this study exhibits the pronounced shortcomings since it is not applicable to the antenna configurations for current BSs such as a uniform rectagular array (URA). In addition, steering null-points in one-dimensional beam space may cause significant gain loss when the nullforming directions are close to the serving direction.


Therefore, in this work, we take into consideration the URA configuration for current BSs and present a novel analog beamforming codebook that has the ability to eliminate sidelobe interference to victim satellite uplink. Additionally, we propose the selection of the codebook over time when multiple satellites are observed in real-life scenarios. To the best of our knowledge, this is the first work that can resolve interference problems by terrestrial BSs when sharing the spectrum between terrestrial and satellite networks.
%\cite{hao2020interference} 
%\cite{tirmizi2022hybrid} 
%\cite{zhu2019cooperative}
%\cite{etsi2013satellite} 
%\textcolor{red}{Need to write more}
%\subsection{Related work}
%\cite{kodheli2020satellite}
%\cite{palacios2022dynamic} 

==> todo.tex <==
\section{To DO}
\begin{itemize}
    \item Sundeep, Gio:  Rewrite the intro
    \item Re-org to put the model and the interference nulling algorithm first, then the simulations
    \item Add a section on elevation angle
    \item In graphs, re-label "SVD" to "no nulling"; "oracle-type nulling" to
    "multi-path nulling" and "tracking-based nulling" to "LOS nulling".
    \item Create a section "Analysis on a LOS Link"
    \item 
    \begin{itemize}
        \item Look at the INR with no nulling conditioned on the 
        elevation angle being in certain bins.
        \item Give an explanation that there are two competing effects:
        slant distance and BS antenna gain
    \end{itemize}
\end{itemize}

